A Sharp Analysis of Model-based Reinforcement Learning with Self-Play

Model-based algorithms -- algorithms that explore the environment through building and utilizing an estimated model -- are widely used in reinforcement learning practice and theoretically shown to achieve optimal sample efficiency for single-agent reinforcement learning in Markov Decision Processes (MDPs). However, for multi-agent reinforcement learning in Markov games, the current best known sample complexity for model-based algorithms is rather suboptimal and compares unfavorably against recent model-free approaches. In this paper, we present a sharp analysis of model-based self-play algorithms for multi-agent Markov games. We design an algorithm -- Optimistic Nash Value Iteration (Nash-VI) for two-player zero-sum Markov games that is able to output an $\epsilon$-approximate Nash policy in $\tilde{\mathcal{O}}(H^3SAB/\epsilon^2)$ episodes of game playing, where $S$ is the number of states, $A,B$ are the number of actions for the two players respectively, and $H$ is the horizon length. This significantly improves over the best known model-based guarantee of $\tilde{\mathcal{O}}(H^4S^2AB/\epsilon^2)$, and is the first that matches the information-theoretic lower bound $\Omega(H^3S(A+B)/\epsilon^2)$ except for a $\min\{A,B\}$ factor. In addition, our guarantee compares favorably against the best known model-free algorithm if $\min \{A,B\}=o(H^3)$, and outputs a single Markov policy while existing sample-efficient model-free algorithms output a nested mixture of Markov policies that is in general non-Markov and rather inconvenient to store and execute. We further adapt our analysis to designing a provably efficient task-agnostic algorithm for zero-sum Markov games, and designing the first line of provably sample-efficient algorithms for multi-player general-sum Markov games.

==> general-CE.tex <==

\section{Learning Learning of CE/CCE in Multiplayer General-sum Games}\label{appendix:multi-CE}

\subsection{Problem formulation}
Let us begin with the definition of a CCE policy of a Markov game. Let $\Acal = \Acal_1 \times \cdots\times \Acal_m$.

\begin{definition}
[CCE in Markov games]\label{defn:CCEpolicy}
	A policy $\pi:=\{ \pi_h(s)\in \Delta_{\Acal}: \ (h,s) \in[H]\times \cS\}$ is a \textbf{CCE} if $\ V^{\dagger,\pi_{-i}}_{h,i}(s) \le V^{\pi}_{h,i}(s)$ for all $(s,h,i)\in\cS\times[H]\times[m]$.
\end{definition}
Compared with a Nash equilibrium, a CEE is not necessarily a product policy, that is, we may not have $\pi_h(s)\in \Delta_{\Acal_1}\times \cdots\times \Delta_{\Acal_m}$. Similar to $\epsilon$-approximate Nash equilibrium, we also define $\epsilon$-approximate CCE.
\begin{definition}[$\epsilon$-approximate CCE in Markov games] \label{def:CCE_multiplayer}
A policy $\pi:=\{ \pi_h(s)\in \Delta_{\Acal}: \ (h,s) \in[H]\times \cS\}$ is an \textbf{$\epsilon$-approximate CCE} if $\max_{i\in[m]}{( V_{1,i}^{\dag, \pi_{-i}}-V_{1,i}^{\pi } )}( s_{1} ) \le \epsilon$.
\end{definition}

Before defining CEs of a Markov game, we need to introduce the concept of strategy modification.

\paragraph{Strategy modification.} A strategy modification $\phi:=\{ \phi_{h,s}(a)\in{ \Acal_i}: \ (h,s,a)\in[H]\times \cS\times \Acal_i\}$ for player $i$ is a set of $S\times H$ injective functions from $\Acal_i$ to itself. 

One can compose a strategy modification $\phi$ with any Markov policy $\pi$ and obtain a  new policy $\phi\circ\pi$ such that when policy $\pi$ chooses to play $\bm{a}:=(a_1,\ldots,a_m)$ at state $s$ and step $h$, policy $\phi\circ\pi$will play $(a_1,\ldots,a_{i-1},\phi_{h,s}(a_i),a_{i+1},\ldots,a_m)$ instead.

\begin{definition}
[CE in Markov games]\label{defn:CEpolicy}
	A policy $\pi:=\{ \pi_h(s)\in \Delta_{\Acal}: \ (h,s) \in[H]\times \cS\}$ is a \textbf{CE} if $\ V^{\phi\circ\pi}_{h,i}(s) \le V^{\pi}_{h,i}(s)$ holds for all strategy modification $\phi$ for player $i$ and for all $(s,h,i)\in\cS\times[H]\times[m]$.
\end{definition}
One can easily verify that if we restrict the choice of strategy modification $\phi$ to those consisting of only constant functions, i.e., $\phi_{h,s}(a)$ being independent of $a$, Definition \ref{defn:CEpolicy} will reduce to the definition of CCE policy.
In addition, any Nash equilibrium is a CE by definition. Since Nash equilibrium always exists, so does CE.

Similarly, we have an approximate version of CE.
\begin{definition}[$\epsilon$-approximate CE in Markov games] \label{def:CE_multiplayer}
A policy $\pi:=\{ \pi_h(s)\in \Delta_{\Acal}: \ (h,s) \in[H]\times \cS\}$ is an \textbf{$\epsilon$-approximate CE} if $\ V^{\phi\circ\pi}_{h,i}(s) - V^{\pi}_{h,i}(s)\le \epsilon$ holds for all strategy modification $\phi$ for player $i$ and for all player $i\in[m]$.
\end{definition}

\subsection{Mutli-player Nash-VI for CE/CCE}

Now equipped with the definition of CEs/CCEs in a Markov game, we are ready to provide the theoretical guarantee of the Multi-\ONASHVI algorithm. The only changes in Algorithm~\ref{alg:Multi-Nash-VI} is that, we change the $\NASH$ Subroutine(Line~\ref{line:general-sum}) to CE/CCE Subroutine respectively.

\begin{theorem}[Multi-\ONASHVI-CCE]
  \label{thm:Multi-Nash-VI-CCE}
There exists an absolute constant $c$, for any $p \in (0, 1]$, let $\iota = \log(SABT /p)$, then with probability at least $1-p$, 
Algorithm~\ref{alg:Multi-Nash-VI} with bonus $\beta_t = c\sqrt{SH^2\iota/t}$ satisfies:
\begin{itemize}
\item $\max_{i\in[m]}{( V_{1,i}^{\dag, \pi^{\text{out}}_{-i}}-V_{1,i}^{\pi^{\text{out}} } )}( s_{1} ) \le \epsilon$, if the number of episodes $K \ge \Omega(H^4S^2 (\prod_{i=1}^m A_i) \iota/\epsilon^2)$.
\item $\Reg(K) = \sum_{k=1}^K \max_{i \in [m]}(V_{1,i}^{\dag, \pi^k_{-i}}-V_{1,i}^{\pi^k } )(s_1) \le  \cO (\sqrt{H^3S^2(\prod_{i=1}^m A_i) T \iota} )$.
\end{itemize}
\end{theorem}

See Appendix~\ref{sec:proof-Multi-Nash-VI-CCE} for the proof. Comparing with Theorem~\ref{thm:Multi-Nash-VI}, the difference is that $\pi^{\text{out}}$ may no longer be a product policy. This is still the case in the following result for CE.

\begin{theorem}[Multi-\ONASHVI-CE]
  \label{thm:Multi-Nash-VI-CE}
There exists an absolute constant $c$, for any $p \in (0, 1]$, let $\iota = \log(SABT /p)$, then with probability at least $1-p$, 
Algorithm~\ref{alg:Multi-Nash-VI} with bonus $\beta_t = c\sqrt{SH^2\iota/t}$ satisfies:
\begin{itemize}
\item $\max_{i\in[m],\phi}{( V_{1,i}^{\phi \circ \pi^{\text{out}}}-V_{1,i}^{\pi^{\text{out}} } )}( s_{1} ) \le \epsilon$, if the number of episodes $K \ge \Omega(H^4S^2 (\prod_{i=1}^m A_i) \iota/\epsilon^2)$.
\item $\Reg(K) = \sum_{k=1}^K \max_{i \in [m],\phi}(V_{1,i}^{\phi \circ \pi^k}-V_{1,i}^{\pi^k } )(s_1) \le  \cO (\sqrt{H^3S^2(\prod_{i=1}^m A_i) T \iota} )$.
\end{itemize}
\end{theorem}

See Appendix~\ref{sec:proof-Multi-Nash-VI-CE} for the proof.
 
% \subsection{Reward-free learning of CE/CCE}
%
% In this section, we show that the outputted empirical transition of Algorithm \ref{alg:multi-VI-zero} can also be used to compute (coarse) correlated equilibriums for the true game, which oftentimes are  more meaningful than Nash equilibriums, especially in games that encourage cooperation.
%
% Now we are ready to present the theoretical guarantee for reward-free learning of CCE. It claims that  
%any CCE of  $\cM(\Phat^{\text{out}},r)$ is also an approximate CCE of the true underlying Markov game $\cM(\P,r)$,
%where $\Phat^{\text{out}}$ is the empirical transition outputted by Algorithm \ref{alg:multi-VI-zero}.
%
%\begin{theorem} \label{thm:multi-rewardfree-CCE} 
%There exists an absolute constant $c$, for any $p \in (0, 1]$, $\epsilon \in (0, H]$, $N \in \N$, if we choose bonus $\beta_t = c\sqrt{ H^2S\iota /t}$ with $\iota = \log(NSABT /p)$ and $K \ge c(H^4 S^2 (\prod_{i=1}^m A_i) \iota/\epsilon^2)$, then with probability at least $1-p$, the output $\Phat^{\text{out}}$ of Algorithm~\ref{alg:multi-VI-zero}
%  has the following property:
%for any $N$ fixed reward functions $r^1,\ldots,r^N$, any CCE of Markov game $\cM(\Phat^{\text{out}}, r^i)$ is also an $\epsilon$-approximate CCE of the true Markov game $\cM(\P,r^i)$ for all $i\in [N]$.
% \end{theorem}
% The proof of Theorem \ref{thm:multi-rewardfree-CCE}  can be found in Appendix \ref{appendix:proof-multi-rewardfree-CCE}. 
%
% Similarly, we also have the theoretical guarantee for reward-free learning of CE. It claims that  
%any CE of  $\cM(\Phat^{\text{out}},r)$ is also an approximate CE of the true underlying Markov game $\cM(\P,r)$,
%where $\Phat^{\text{out}}$ is the empirical transition outputted by Algorithm \ref{alg:multi-VI-zero}.
%
%\begin{theorem} \label{thm:multi-rewardfree-CE} 
%There exists an absolute constant $c$, for any $p \in (0, 1]$, $\epsilon \in (0, H]$, $N \in \N$, if we choose bonus $\beta_t = c\sqrt{ H^2S\iota /t}$ with $\iota = \log(NSABT /p)$ and $K \ge c(H^4 S^2 (\prod_{i=1}^m A_i) \iota/\epsilon^2)$, then with probability at least $1-p$, the output $\Phat^{\text{out}}$ of Algorithm~\ref{alg:multi-VI-zero}
%  has the following property:
%for any $N$ fixed reward functions $r^1,\ldots,r^N$, any CE of Markov game $\cM(\Phat^{\text{out}}, r^i)$ is also an $\epsilon$-approximate CE of the true Markov game $\cM(\P,r^i)$ for all $i\in [N]$.
% \end{theorem}
% The proof of Theorem \ref{thm:multi-rewardfree-CE}  can be found in Appendix \ref{appendix:proof-multi-rewardfree-CE}. 
%
%








 
 
 

==> general-free.tex <==



\subsection{Reward-free VI for multi-player general-sum Markov games}


\begin{algorithm}[t]
   \caption{Reward-free VI for multi-player general-sum games: Exploration Phase}
   \label{algorithm:Reward-free-exploration-general}
\begin{algorithmic}[1]
   \STATE {\bfseries Initialize:} for any $(s, \bm{a}, h,k)$,
   ${\Vt}_{H+1}^k(s,\bm{a})\setto 0$, $N_{h}(s,\bm{a})\setto 0$,
   $\widehat{\P}_h^k(\cdot|s, \bm{a})\setto {\rm Uniform}(\cS)$.
   \FOR{episode $k=1,\dots,K$}
   \FOR{step $h=H,H-1,\dots,1$}
   \FOR{$(s, \bm{a})\in\cS\times\cA$}
   \STATE $t \setto N_{h}(s, \bm{a})$.
   \IF{$t>0$}
   \STATE $\beta_t \setto \sqrt{ H^2S\iota /t}$
   and $\widehat{\P}_h^k(\cdot|s,\bm{a})\setto N_h(s, \bm{a}, \cdot)/t$.
   \STATE $\Qt_{h}^k(s, \bm{a})\setto \min\{
   [\widehat{\P}_{h}^k {\Vt}_{h+1}^k](s, \bm{a}) + \beta_t, H\}$.
   \ENDIF
   \ENDFOR
   \FOR{$s \in \cS$}
   \STATE $\pi_h(s) \setto \arg\max_{\bm{a}\in \cA} \Qt_{h}^k(s, \bm{a})$
   and $\Vt_h^k(s) \setto \max_{\bm{a}\in \cA} \Qt_{h}^k(s, \bm{a})$.
   \ENDFOR
   \ENDFOR
   \FOR{step $h=1,\dots, H$}
   \STATE Take action $\bm{a}_h \setto  \pi_h(s_h)$ and observe $s_{h+1}$. 
   \STATE $N_{h}(s_h, \bm{a}_h)\setto N_{h}(s_h, \bm{a}_h) + 1$.
   \STATE $N_h(s_h, \bm{a}_h, s_{h+1}) \setto N_h(s_h, \bm{a}_h, s_{h+1})
   + 1$.
   \ENDFOR
   \ENDFOR
   \vspace{1mm}
  \STATE {\bfseries Output} $\Phat^{k^\star} \setto \{\Phat_h^{k^\star}(\cdot\mid s,\bm{a})\}_{(h,s,\bm{a})\in[H]\times\cS\times\cA}$ where 
  $k^\star = \arg\min_{k\in[K]} \Vt^k_1(s_1)$.
\end{algorithmic}
\end{algorithm}


We can also generalize the reward-free value-iteration algorithm (Algorithm \ref{algorithm:Reward-free-exploration}) to the multi-player general-sum setting by using a larger bonus $\beta_t = \sqrt{ H^2S\iota /t}$. 
This is the only key difference between Algorithm \ref{algorithm:Reward-free-exploration-general} and
Algorithm \ref{algorithm:Reward-free-exploration}.


Similarly, we have the following theoretical guarantee for Algorithm \ref{algorithm:Reward-free-exploration-general}.
\begin{theorem}\label{thm:rewardfree-explore-general}
Let $r^1,\ldots,r^N$ be $N$ reward functions chosen independent of the randomness induced by running Algorithm \ref{algorithm:Reward-free-exploration}.
 For any $p \in (0,1]$, choose the exploration bonus $\beta_t$ as in Algrothm~\ref{algorithm:Reward-free-exploration-general} for $\iota = C\log(SABHTN/p)$ with large absolute constant $C$. Then, with probability at least $1-p$, for all $s\in\cS$, $k\in[K]$, $i\in[M]$, $n \in[N]$ and $\pi^{kn}$ that is a Nash-equilibrium policy for $\widehat{\cM}^{k,n} := (\Phat^k,r^n)$,
$$V_{h,i}^{\pi^{kn}_{-i},\dagger}(s) - V_{h,i}^{\pi^{kn}}(s) \le \cO\paren{\Vt_{h}^k(s)}.$$
 \end{theorem}
 
 
 
 Theorem \ref{thm:rewardfree-explore-general} shows that 
 the improvement that any player can achieve by unilaterally changing her own policy is upper bounded by the corresponding exploration uncertainty $\Vt_1^k(s_1)$ up to a constant factor. 
 
Since Algorithm \ref{algorithm:Reward-free-exploration-general} can be viewed as a zero-reward version of UCB-VI with a larger exploration bonus, one can easily adapt the analysis of \cite{azar2017minimax} and give the following guarantee.
\begin{theorem}[UCB-VI with larger bonus]\cite{azar2017minimax} \label{thm:UCB-VI-general}
For any $p \in (0,1]$, choose the exploration bonus $\beta_t$ as in Algrothm~\ref{algorithm:Reward-free-exploration-general} for $\iota = C\log(TNSH \prod_{i=1}^{M}A_i /p)$ with large absolute constant $C$. Then, with probability at least $1-p$, 
$$ \sum_{k=1}^{K} \Vt_{1,i}^k(s_1) \le \cO\paren{S\sqrt{KH^4\iota\prod_{i=1}^{M}A_i}+H^3S^2\iota\prod_{i=1}^{M}A_i}.$$
\end{theorem}

By combining Theorem \ref{thm:rewardfree-explore-general} with
Theorem \ref{thm:UCB-VI-general}, we obtain the sample efficiency of Algorithm \ref{algorithm:Reward-free-exploration-general}.

\begin{corollary}\label{cor:rewardfree-samplecomplex}
	For any $p \in (0,1]$, choose the exploration bonus $\beta_t$ as in Algrothm~\ref{algorithm:Reward-free-exploration-general} for $\iota = C\log(TNSH\prod_{i=1}^{M}A_i /p)$ with large absolute constant $C$. 
	If we choose $K$ s.t.
	$$
K \ge \Omega\paren{\frac{H^4S^2(\prod_{i=1}^{M}A_i)\iota }{\epsilon_{\rm explore}^2} + \frac{H^3S^2 (\prod_{i=1}^{M}A_i)\iota}{\epsilon_{\rm explore}}},
$$ 
then, with probability at least $1-p$, for all $n\in[N]$ and $\pi^{n}$ that is Nash-equilibrium for $\widehat{\cM}^{k^\star,n} := (\Phat^{k^\star},r^n)$,
	$$\max_{i\in[M]}\paren{V_{1,i}^{\pi^n_{-i},\dagger}(s_1) - V_{1,i}^{\pi^n}(s_1) }\le \epsilon_{\rm explore}.$$
\end{corollary}

Therefore, $\Omega(H^4S^2(\prod_{i=1}^{M}A_i)\iota/\epsilon^2)$ episodes suffice for learning $\epsilon$-Nash policies for all $N$ reward functions simultaneously.
Note that the sample complexity here is quadratic in the number of states.
This sub-optimality arises from using the exploration bonus $\beta_t = \sqrt{ H^2S\iota /t}$ that is  larger than usual by an $\sqrt{S}$ factor. 












==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> opt_VI.tex <==
%!TEX root = main.tex
\newcommand{\Va}{\mathbb{V}}
\newcommand{\Vahat}{\widehat{\mathbb{V}}}

\newcommand{\Vdstar}{V^{\star}}
\newcommand{\Qdstar}{Q^{\star}}

\newcommand{\VpikA}{V^{\dagger,\nu^k}}
\newcommand{\VpikB}{V^{\mu^k,\dagger}}
\newcommand{\QpikA}{Q^{\dagger,\nu^k}}
\newcommand{\QpikB}{Q^{\mu^k,\dagger}}

\newcommand{\Vpik}{V^{\pi^k}}
\newcommand{\Qpik}{Q^{\pi^k}}

\section{Value Iteration with Optimism} \label{sec:VI}

In this section, we present the our algorithm Optimistic Value Iteration for Markov Games (Nash-VI) and the corresponding regret guarantee. 


\subsection{Algorithm description}
The general idea behind Nash-VI (Algorithm~\ref{algorithm:Nash-VI}) is similar to VI-ULCB, but with
\begin{itemize}
   \item a new design of the optimistic bonus, which enables the algorithm to achieve minimax regret rate w.r.t. to $S$ and $H$.
   \item a different computational scheme to find the equalibirum, which enables the algorithm to run in polynomial time.  
\end{itemize}

We will first briefly go through the general idea, then focus on the two points mentioned above.

Our algorithm is based on value iteration. To efficiently explore the environment, optimism bonuses are added to the Q-values estimated from past obervations as in \cite{azar2017minimax}. However, when selecting the policy based on the Q-values, instead of choosing the maximum directly ("greedy"), we have to compute the equalibrium ("jointly greedy"). This is because in zero sum games, the two players have conflicting goals. Therefore, when maximizing one player's utility, she has to be aware of the fact that the other player is also trying to minimizing her utility and choose the equalibirum.

\paragraph{Tighter Bonus.} To see why the new bonus can achieve better regret rate, let's compare the optimistic Hoeffding bonus in Nash-VI (Algorithm~\ref{algorithm:Hoeffding-Bonus}) $\beta_t = C\sqrt{H^2\iota/t}$ and the optimistic bonus in VI-ULCB (Algorithm 1 in \cite{bai2020provable}) $\beta_t = C\sqrt{SH^2\iota/t} $ where $\iota = \log(SABKH/p)$ is the logarithmic factor and $\widehat{\Va}_hV(s,a,b) :=\Var_{s'\sim \Phat_h(\cdot|s,a,b)}V(s') $ is the empirical variance estimator. It's clear in the new bonus design we don't have the $\sqrt{S}$ factor anymore. The $S$ factor comes from a uniform concentration in $L^1$ norm when upper bounding the best response (Lemma 12 in \cite{bai2020provable}). However, this uniform bound is too restrictive and not necessary. 

To guarantee the $\up{Q}$ and $\low{Q}$ are still upper and lower bounds of true Q-value under best response, we add a new term $\widehat{\P}^k_h (\up{V}_{h+1} - \low{V}_{h+1})(s, a, b)/H$ in Line~\ref{line:Qup} and Line~\ref{line:Qlow}. In Lemma~\ref{lem:sandwichVstar} and Lemma~\ref{lem:sandwichVpik}, we will prove this will suffice and the new term $\widehat{\P}^k_h (\up{V}_{h+1} - \low{V}_{h+1})(s, a, b)/H$ term is of order $\cO(\sqrt{H\iota/t})$ in average. Therefore, we can remove the $\sqrt{S}$ factor in the bonus. Similar technique has been used in \cite{dann2019policy} to construct policy certificate in an MDP.

\paragraph{Bernstein Concentration.} We also design a bonus based on Bernstein-type concentration in Algorithm~\ref{algorithm:Bernstein-Bonus}. Comparing with the Hoeffding-type bound, the Bernstein-type bonus is of order $\cO(\sqrt{H\iota/t})$ in average (See the proof of Theorem~\ref{thm:Nash-VI}), and thus spare a $\sqrt{H}$ factor. Using Bernstein concentration to improve regret rate is a popular technique in RL literature, first appears in \cite{azar2017minimax} to achieve the minimax dependence on $H$. 

\paragraph{Coarse Correlated Equalibirum (CCE).} When we add optimistic bonus to the Q-value, the corresponding matrix game becomes a general-sum one and finding the Nash equalibirum is PPAD-hard \cite{daskalakis2013complexity}. To overcome this computational challenge, we find a Coarse Correlated Equalibirum (CCE) instead, which is first introduced in \cite{xie2020learning} to solve Markov Games with value iterations. CCE always exist, can be computed with linear programming in polynomial time, and the returned policy $\pi \setto \CCE (\up{Q}(\cdot, \cdot), \low{Q}(\cdot, \cdot))$ we have
$$
\E_{(a,b)\sim \pi}\up{Q}(a,b) \ge \max_{a^{\star}}\E_{(a,b)\sim \pi}\up{Q}(a^{\star},b), \,\,\,\, \E_{(a,b)\sim \pi}\low{Q}(a,b) \le \min_{b^{\star}}\E_{(a,b)\sim \pi}\low{Q}(a,b^{\star}).
$$

In the following we will use $\mu$ and $\nu$ to denoe the marginal distribution of $\pi$. Since $\pi$ may be a correlated policy (otherwise we get the Nash equalibirum directly), $V^{\mu,\nu}$ can be very different from $V^{\pi}$.


\begin{algorithm}[t]
   \caption{Optimistic Nash Value Iteration for Markov Games (Nash-VI)}
   \label{algorithm:Nash-VI}
\begin{algorithmic}[1]
   \STATE {\bfseries Initialize:} for any $(s, a, b, h)$,
   $\up{Q}_{h}(s,a, b)\setto H$, $\low{Q}_{h}(s,a, b)\setto 0$,
   $N_{h}(s,a, b)\setto 0$.
   \FOR{episode $k=1,\dots,K$}
   \STATE Receive $s_1$.
   \FOR{step $h=H,H-1,\dots,1$}
   \FOR{$(s, a, b)\in\cS\times\cA\times \cB$}
   \STATE $t \setto N_{h}(s, a, b)$;
   \IF{$t>0$}
   \STATE $\beta_t \setto {\sf Bonus}(t,S,H,\widehat{\Va}_h \up{V}_{h+1}(s,a,b),\iota)$
   \STATE $\up{Q}_{h}(s, a, b)\setto \min\{(r_h +
   \widehat{\P}_{h} \up{V}_{h+1})(s, a, b) +  C\widehat{\P}_h (\up{V}_{h+1} - \low{V}_{h+1})(s, a, b)/H +
   \beta_t, H\}$ \label{line:Qup}
   \STATE $\low{Q}_{h}(s, a, b)\setto \max\{(r_h +
   \widehat{\P}_{h} \low{V}_{h+1})(s, a, b) - C\widehat{\P}_h (\up{V}_{h+1} - \low{V}_{h+1})(s, a, b)/H
   - \beta_t, 0\}$ \label{line:Qlow}
   \ENDIF
   \ENDFOR
   \FOR{$s \in \cS$}
   \STATE $\pi_h(\cdot, \cdot|s) \setto \CCE (\up{Q}_h(s, \cdot, \cdot), \low{Q}_h(s, \cdot, \cdot))$
   \STATE $\up{V}_h(s) \leftarrow (\D_{\pi_h}\up{Q}_h)(s); \quad \low{V}_h(s) \leftarrow (\D_{\pi_h} \low{Q}_h)(s)$.
   \ENDFOR
   \ENDFOR
   \FOR{step $h=1,\dots, H$}
   \STATE Take action $(a_h, b_h) \sim  \pi_h(\cdot, \cdot| s_h)$.
   \STATE Observe reward $r_h$ and next state
   $s_{h+1}$. 
   \STATE $N_{h}(s_h, a_h, b_h)\setto N_{h}(s_h, a_h, b_h) + 1$.
   \STATE $N_h(s_h, a_h, b_h, s_{h+1}) \setto N_h(s_h, a_h, b_h, s_{h+1})
   + 1$.
   \STATE $\widehat{\P}_h(\cdot|s_h, a_h,
     b_h)\setto N_h(s_h, a_h, b_h, \cdot)/N_h(s_h, a_h, b_h)$.
   \ENDFOR
   \ENDFOR
\end{algorithmic}
\end{algorithm}

\begin{algorithm}[h]
   \caption{Hoeffding-Bonus}
   \label{algorithm:Hoeffding-Bonus}
\begin{algorithmic}[1]
   \STATE {\bfseries Require:} $t,S,H,\iota$.
   \STATE $\beta \setto C\sqrt{H^2\iota/t}$
   \RETURN $\beta$
\end{algorithmic}
\end{algorithm}

\begin{algorithm}[h]
   \caption{Bernstein-Bonus}
   \label{algorithm:Bernstein-Bonus}
\begin{algorithmic}[1]
   \STATE {\bfseries Require:} $t,S,H,\widehat{\Va}_h \up{V}_{h+1}(s,a,b),\iota$.
   \STATE $\beta \setto C(\sqrt{\iota\widehat{\Va}_h \up{V}_{h+1}(s,a,b)/t} + H^2S\iota/t )$
   \RETURN $\beta$
\end{algorithmic}
\end{algorithm}

\subsection{Analysis}
We now present the main result of this section. We denote $\pi^k$, $\mu^k$ and $\nu^k$ to denote the policies at the beginning of the $k$-th episode.


\begin{theorem}[Regret of Nash-VI]
   \label{thm:Nash-VI}
   For any $p \in (0,1]$, choose the Hoeffding-type bonus $\beta_t$ as in Algrothm~\ref{algorithm:Hoeffding-Bonus} for large absolute constant $C$ and $\iota = \log(SABT /p)$. Then, with probability $1-p$, Nash-VI (Algorithm~\ref{algorithm:Nash-VI}) achieves regret
      $$
\sum_k (\VpikA_1(s_1^k) - \VpikB_1(s_1^k)) \le  \cO \paren{\sqrt{H^3SABT\iota} + H^3S^{3/2}AB\iota^2 }.
$$
If we use Bernstein-type bonus $\beta_t$ as in Algrothm~\ref{algorithm:Bernstein-Bonus} instead, Nash-VI (Algorithm~\ref{algorithm:Nash-VI}) achieves regret
$$
\sum_k (\VpikA_1(s_1^k) - \VpikB_1(s_1^k)) \le  \cO \paren{\sqrt{H^2SABT\iota} + H^3S^{3/2}AB\iota^2 }.
$$
\end{theorem}

\paragraph{Transition to PAC bound} By a standard online-to-batch conversion (for example, A.2 in \cite{bai2020provable}), out regret guarantee immediately implies the sample complexity guarantee. 
\begin{corollary}
Suppose the initial state of the Markov Game is fixed at $s_1$ and we sample $\hat{\mu} \sim \{\mu^k\}_{k=1}^K$ and $\hat{\nu} \sim \{\nu^k\}_{k=1}^K$. Then with probability $1-p$, if we run Nash-VI (Algorithm~\ref{algorithm:Nash-VI}) with Hoeffding type bonus (Algrothm~\ref{algorithm:Hoeffding-Bonus}) for $K$ episodes with
$$
K \ge \Omega(\frac{H^4SAB\iota}{\epsilon^2}+\frac{H^3S^{3/2}AB\iota^2}{\epsilon}),
$$  
its induced policies $(\hat{\mu},\hat{\nu})$ will be $\epsilon$-approximate Nash, i.e., $V_1^{\dagger,\hat{\nu}}(s_1) - V_1^{\hat{\mu},\dagger}(s_1) \le \epsilon$.

If we use Bernstein-type bonus (Algrothm~\ref{algorithm:Bernstein-Bonus}) instead, 
$$
K \ge \Omega(\frac{H^3SAB\iota}{\epsilon^2}+\frac{H^3S^{3/2}AB\iota^2}{\epsilon}),
$$
will suffice.
\end{corollary}

\paragraph{Comparison with existing work.} Comparing with the lower bound \cite{jin2018q,bai2020provable}, both the regret and the sample complexity are minimax optimal w.r.t. $T$ (or $\epsilon$), $S$ and $H$ up to logarithmic factors. This significantly improves the result in \cite{bai2020provable,xie2020learning}.

The only gap in sample complexity between our result and the lower bound is in the dependence of $A$ and $B$. While the lower bound is $\Omega(A+B)$, we have $\tlO(AB)$. The Nash V-learning algorithm \cite{bai2020near} indeed achieves the $\tlO(A+B)$ rate, but the dependence on $H$ is much worse and the output policy is a nested mixture, which is hard to implement. It remains an interesting open question whether we can take the advantage of both approach to achieve simple policy with optimal dependence in all key parameters.

\paragraph{Connection to reward-free exploration}









==> proof_exp1.tex <==
% !TEX root = main.tex

\section{Proof of Theorem~\ref{thm:exp1}}
\label{appendix:pf_exp1}


\paragraph{Notation:} To be clear from the context, we denote the
upper bound and lower bound $\up{Q}$ and $\low{Q}$ computed at the
$k$-th episode as $\up{Q^k}$ and $\low{Q^k}$, and policies
computed and used at the $k$-th episode as $\pi^k$. We denote the marginal distribution of randomized policy $\pi^k$ on two players as $\mu^k$ and $\nu^k$. 

\paragraph{Choice of bonus:} $\beta_t = c\sqrt{SH^2\iota/t}$ for sufficient large absolute constant $c$.

\begin{lemma}[ULCB]\label{lem:ULCB_sim}
With probability at least $1-p$, we have following bounds for any $(s, a, b, h, k)$:
% $\in \cS\times\cA\times\cB\times[H]\times[K]$
\begin{align}
&\up{V_h^k}(s) \ge V_h^{\dagger, \nu^k}(s),  &\up{Q_h^k}(s, a, b) \ge&  Q_h^{\dagger, \nu^k}(s, a, b) \label{eq:ucb_sim}\\
&\low{V_h^k}(s) \le V_h^{\mu^k, \dagger}(s), &\low{Q_h^k}(s, a, b) \le& Q_h^{\mu^k, \dagger}(s, a, b) \label{eq:lcb_sim}
\end{align}
\end{lemma}
\begin{proof}
By symmetry, we only need to prove the statement \eqref{eq:ucb_sim}. For each fixed $k$, we prove this by induction from $h=H+1$ to $h=1$. For base case, we know at the $(H+1)$-th step, 
$\up{V_{H+1}^k}(s) = V_{H+1}^{\dagger, \nu^k}(s) = 0$.

Now, assume the left inequality in \eqref{eq:ucb_sim} holds for $(h+1)$-th step, for the $h$-th step, we first recall the updates for $Q$ functions respectively:
\begin{align*}
\up{Q_{h}^k}(s, a, b) = & \min\set{(r_h +
   \widehat{\P}_{h}^k \up{V_{h+1}^k})(s, a, b) +
   \beta_t, H}\\
 Q_h^{\dagger, \nu^k}(s, a, b)
=& (r_h + \P_{h} V_{h+1}^{\dagger, \nu^k})(s, a, b)
\end{align*}
In case of $\up{Q_{h}^k}(s, a, b) = H$, the right inequality in \eqref{eq:ucb_sim} clearly holds. Otherwise, we have:
\begin{align*}
\up{Q_{h}^k}(s, a, b) - Q_h^{\dagger, \nu^k}(s, a, b)
=& [\widehat{\P}_{h}^k \up{V_{h+1}^k}](s, a, b) - [\P_{h} V_{h+1}^{\dagger, \nu^k}](s, a, b) +  \beta_t\\
=& [\widehat{\P}_{h}^k (\up{V_{h+1}^k} - V_{h+1}^{\dagger, \nu^k})](s, a, b) - [(\widehat{\P}_{h}^k -\P_{h}) V_{h+1}^{\dagger, \nu^k}](s, a, b) +  \beta_t
\end{align*}
Since $\widehat{\P}_{h}^k$ perserves the positivity, by induction assumption, we know the first term is positive. By Lemma \ref{lem:uniform_concern_sim}, we know the second term $\ge -\beta_t$. This finishes the proof of the right inequality in \eqref{eq:ucb_sim}.

To prove the left inequality in \eqref{eq:ucb_sim}, again recall the updates for $V$ functions respectively:
\begin{align*}
  \up{V_{h}^k}(s) =
  & (\D_{\pi^k_h} \up{Q_h^k})(s) \ge \sup_{\mu \in \Delta_\cA} (\D_{\mu \times \nu^k_h} \up{Q_h^k})(s), \\ 
  V_h^{\dagger, \nu^k}(s) =  &\sup_{\mu \in \Delta_\cA}   (\D_{\mu \times \nu^k_h} Q_h^{\dagger, \nu^k})(s).
\end{align*}
where the first equation is by the definition of policy $\pi^k$ is CCE. Therefore:
\begin{equation*}
\up{V_{h}^k}(s) - V_h^{\dagger, \nu^k}(s)
\ge \sup_{\mu \in \Delta_\cA}[\D_{\mu \times \nu^k_h} (\up{Q_h^k} - Q_h^{\dagger, \nu^k})](s) \ge 0.
\end{equation*}
This finishes the proof.
\end{proof}

\begin{lemma}[Uniform Concentration]\label{lem:uniform_concern_sim}
  Consider value function class
  \begin{equation*}
    \mathcal{V}_{h+1} =
    \set{V:\cS_{h+1}\to\R~\mid~V(s)\in[0,H]~\textrm{for
        all}~s\in \cS_{h+1}}.
    % \mathcal{V} = \set{V: \cS\times\cA\times\cB \rightarrow \R : V(s,
    %   a, b)\in[0, H]~\textrm{for all}~(s,a,b)}.
  \end{equation*}
  % Suppose we have encountered $(s, a, b)$ for $t$ times, and $\hat{\P}$ is the empirical transition matrix. Then, 
  There exists an absolute constant $c$, with probability at least $1-p$, we have:
  \begin{equation*}
    \abs{[(\hat{\P}^k_h - \P_h)V](s, a, b)} \le
    c\sqrt{SH^2\iota/N^k_h(s, a, b)} \quad \textrm{for all}~ (s, a, b,
    k, h) ~\textrm{and all}~ V\in \mathcal{V}_{h+1}. 
  \end{equation*}
\end{lemma}
\begin{proof}
By standard concentration argument. See \cite{bai2020provable}.
\end{proof}

\begin{proof}[Proof of Theorem \ref{thm:exp1}]
By Lemma \ref{lem:ULCB_sim}, we know the regret,
\begin{equation*}
\text{Regret}(K) \le \sum_{k=1}^K \left[V^{\dagger, \nu^k}_1 (s_1) - V^{\mu^k, \dagger}_1 (s_1)\right] 
\le \sum_{k=1}^K [\up{V_1^k}(s_1)  - \low{V_1^k}(s_1)].
\end{equation*}
On the other hand, by the updates in Algorithm \ref{algorithm:ucbvi_sim}, we have:
\begin{align*}
[\up{V_h^k} - \low{V_h^k}](s^k_h)
=& [\D_{\pi^k_h} (\up{Q_h^k} - \low{Q_h^k})](s^k_h), \\
=& [\up{Q_h^k} - \low{Q_h^k}](s^k_h, a^k_h, b^k_h) + \xi^k_h\\
\le & [\widehat{\P}_{h}^k (\up{V_{h+1}^k} - \low{V_{h+1}^k})](s^k_h, a^k_h, b^k_h) + 2\beta_h^k + \xi_h^k \\
\le & \P (\up{V_{h+1}^k} - \low{V_{h+1}^k})](s^k_h, a^k_h, b^k_h) + 4\beta_h^k + \xi_h^k\\
= & [\up{V_{h+1}^k} - \low{V_{h+1}^k})](s^k_{h+1}) + 4\beta_h^k + \xi_h^k + \zeta_h^k
\end{align*}
the last inequality is due to Lemma \ref{lem:uniform_concern_sim}. $\xi_h^k$ and $\zeta_h^k$ are defined as
\begin{align*}
\xi_h^k =& [\D_{\mu^k_h\times \nu^k_h}(\up{Q_h^k} - \low{Q_h^k})](s^k_h)  - [\up{Q_h^k} -
           \low{Q_h^k}](s^k_h, a^k_h, b^k_h)\\ 
\zeta_h^k =& 
             [\P_h(\up{V_{h+1}^k} - \low{V_{h+1}^k})](s^k_h, a^k_h, b^k_h) -
             [\up{V_{h+1}^k} - \low{V_{h+1}^k}](s^k_{h+1}) 
\end{align*}
Both $\xi_h^k$ and $\zeta_h^k$ are martingale difference sequence,
therefore by the Azuma-Hoeffding inequality we have with probability
$1-p$ that
\begin{equation*}
  \sum_{k, h} \xi_h^k \le \cO(\sqrt{HT\iota}) \quad {\rm and} \quad
  \sum_{k, h} \zeta_h^k \le \cO(\sqrt{HT\iota}). 
\end{equation*}
Therefore, by our choice of bonus $\beta_t$ and the Pigeonhole
principle, we have
\begin{align*}
  & \quad \sum_{k=1}^K \brac{\up{V_1^k}(s_1)  - \low{V_1^k}(s_1)}
    \le \sum_{k, h} \paren{4\beta^k_h + \xi^k_h + \zeta^k_h} \le c\cdot \sum_{h,s,a,b} 
    \sum_{t=1}^{N^K_h(s,a,b)} \sqrt{\frac{H^2S\iota}{t}} + \cO(\sqrt{HT\iota}) \\
  & = \sum_{h,s,a,b}  \cO\paren{\sqrt{H^2S\iota
    \cdot N^K_h(s, a, b)}} + \cO(\sqrt{HT\iota}) \le
    \cO\paren{\sqrt{H^3S^2ABT\iota}}.
\end{align*}
This finishes the proof.
\end{proof}


==> result_multi_short.tex <==
%\section{Multi-player general-sum games}
%\label{section:multi-player-short}

%We adapt our analysis to multi-player general-sum games and present the first lines of provably efficient algorithms. Concretely, we design two model-based algorithms Multi-Nash-VI and Multi-VI-Zero (Algorithm~\ref{alg:Multi-Nash-VI} and Algorithm \ref{alg:multi-VI-zero}) that can find an ($\epsilon$-approximate) \{\NASH,~\CE,~\CCE\} equilibrium for any multi-player general-sum Markov game in $\tlO(H^4S^2\prod_{i=1}^m A_i/\epsilon^2)$ episodes of game playing, where $A_i$ is the number of actions for player $i\in\set{1,\dots,m}$ (Theorem~\ref{thm:Multi-Nash-VI} and Theorem \ref{thm:multi-rewardfree-explore}). Due to space limit, we defer the detailed setups, algorithms and results to Appendix~\ref{sec:multi}. 



==> reward-free.tex <==
%!TEX root = main.tex
\section{Reward-free Exploration} \label{sec:reward-free}

\newcommand{\Qexp}{{\bar{Q}^k}}
\newcommand{\Vexp}{{\bar{V}^k}}



\newcommand{\Qpih}{Q^{\pihat_k}}
\newcommand{\Vpih}{V^{\pihat_k}}
\newcommand{\pit}{{\tilde{\pi}}}

\newcommand{\Mcal}{\mathcal{M}}
\newcommand{\Acal}{\mathcal{A}}
\newcommand{\Mfrak}{\mathfrak{M}}

\newcommand{\nuhat}{\hat{\nu}}
\newcommand{\muhat}{\hat{\mu}}


\begin{algorithm}[t]
   \caption{Reward-free Value Iteration for Markov Games: Exploration Phase}
   \label{algorithm:Reward-free-exploration}
\begin{algorithmic}[1]
   \STATE {\bfseries Initialize:} for any $(s, a, b, h,k)$,
   ${\Vt}_{H+1}^k(s,a, b)\setto 0$, $N_{h}(s,a, b)\setto 0$,
   $\widehat{\P}_h^k(\cdot|s, a,b)\setto {\rm Uniform}(\cS)$.
   \FOR{episode $k=1,\dots,K$}
   \FOR{step $h=H,H-1,\dots,1$}
   \FOR{$(s, a, b)\in\cS\times\cA\times \cB$}
   \STATE $t \setto N_{h}(s, a, b)$.
   \IF{$t>0$}
   \STATE $\beta_t \setto \sqrt{ H^2\iota /t}+ {H^2S\iota}/t$
   and $\widehat{\P}_h^k(\cdot|s, a,
     b)\setto N_h(s, a, b, \cdot)/t$.
   \STATE $\Qt_{h}^k(s, a, b)\setto \min\{
   [\widehat{\P}_{h}^k {\Vt}_{h+1}^k](s, a, b) + \beta_t, H\}$.
   \ENDIF
   \ENDFOR
   \FOR{$s \in \cS$}
   \STATE $\pi_h(s) \setto \arg\max_{(a,b)\in \cA\times\cB} \Qt_{h}^k(s, a, b)$
   and $\Vt_h^k(s) \setto \max_{(a,b)\in \cA\times\cB} \Qt_{h}^k(s, a, b)$.
   \ENDFOR
   \ENDFOR
   \FOR{step $h=1,\dots, H$}
   \STATE Take action $(a_h, b_h) \setto  \pi_h(s_h)$ and observe $s_{h+1}$. 
   \STATE $N_{h}(s_h, a_h, b_h)\setto N_{h}(s_h, a_h, b_h) + 1$.
   \STATE $N_h(s_h, a_h, b_h, s_{h+1}) \setto N_h(s_h, a_h, b_h, s_{h+1})
   + 1$.
   \ENDFOR
   \ENDFOR
   \vspace{1mm}
  \STATE {\bfseries Output} $\Phat^{k^\star} \setto \{\Phat_h^{k^\star}(\cdot\mid s,a,b)\}_{(h,s,a,b)\in[H]\times\cS\times\cA\times\cB}$ where 
  $k^\star = \arg\min_{k\in[K]} \Vt^k_1(s_1)$.
\end{algorithmic}
\end{algorithm}

\begin{algorithm}[t]
   \caption{Reward-free Value Iteration for Markov Games: Planning Phase}
   \label{algorithm:Reward-free-planning}
\begin{algorithmic}[1]
   \STATE {\bfseries Input}: model $\widehat{\cM}= (\Phat,r)$, accuracy $\epsilon$.
    \STATE {\bfseries Initialize:} for any $(s, a, b, h)$,
   ${V}_{H+1}(s,a, b)\setto 0$.
 \FOR{step $h=H,H-1,\dots,1$}
   \FOR{$(s, a, b)\in\cS\times\cA\times \cB$}
   \STATE $Q_{h}(s, a, b)\setto 
   [\widehat{\P}_{h} {V}_{h+1}](s, a, b) + r_h(s,a,b)$.
   \ENDFOR
   \FOR{$s \in \cS$}
   \STATE $(\muhat_h(\cdot\mid s),\nuhat_h(\cdot\mid s)) \setto \mbox{NASH-ZERO-SUM}(Q_{h}(s, \cdot, \cdot),\epsilon)$.
   \STATE $V_h(s) \setto \muhat_h(\cdot \mid s)^\top Q_{h}(s, \cdot, \cdot) \nuhat_h(\cdot \mid s)$.
   \ENDFOR
   \ENDFOR
   \STATE {\bfseries Output} $(\muhat,\nuhat)\setto \{(\muhat_h(\cdot\mid s),\nuhat_h(\cdot\mid s))\}_{(h,s)\in[H]\times\cS}.$
\end{algorithmic}
\end{algorithm}


In this section, we present our algorithm Reward-free Value Iteration for Markov Games, along with its sample efficiency guarantee. 

\subsection{Algorithms}

Our algorithm consists of two phases: the reward-free exploration phase and the planning phase. 

\paragraph{Exploration phase.} Algorithm \ref{algorithm:Reward-free-exploration} can be viewed as a zero-reward version of UCB-VI \cite{azar2017minimax}. 
Specifically, it can be derived by setting the reward function in UCB-VI to be zero and keeping all remaining parts unchanged. 
As a result, the exploration is purely driven by the bonus function. 

Note that in Algorithm \ref{algorithm:Reward-free-exploration}, the value functions $\Qt$ is clearly no longer an upper bound for the optimal value function as in \cite{azar2017minimax}. Instead, one should intuitively think of it as a measure of model estimation uncertainty. To be more specific, $\Qt_h(s,a,b)$ quantifies the uncertainty (suboptimality) the agent may suffer if it starts from taking action $(a,b)$ in state $s$ at step $h$ and making decisions by utilizing the empirical estimate $\Phat$ in the remaining steps. 
A rigorous version of this argument will be given in Theorem \ref{thm:rewardfree-explore}.

\paragraph{Planning phase.} After $K$ episodes, Algorithm \ref{algorithm:Reward-free-exploration} will output an estimate of the model transition $\Phat$, which together with the target reward function $r$ will be the input of our planning phase. Here, Algorithm \ref{algorithm:Reward-free-planning} simply calculates an approximate Nash equilibrium for the estimated MDP 
$\widehat{\cM} := (\Phat,r)$, assuming access to a computation oracle NASH-ZERO-SUM that can compute an $\epsilon$-approximate Nash-equilibrium for any matrix game of size $A\times B$.
NASH-ZERO-SUM can be easily implemented with Mirror Descent, with total computation complexity $\tilde{\cO}(AB/\eps^2)$,
which can be further improved to $\tilde{\cO}(AB/\eps)$ by incorporating Nesterov's acceleration technique \cite{krichene2015accelerated}. 





\subsection{Theoretical guarantees}

Now we are ready to present the theoretical guarantees for our algorithms, along with an almost matching lower bound for the sample complexity of reward-free Markov games.

\subsubsection{Exploration phase guarantees}

Before stating the main theorem, we introduce the following definition of $\epsilon$-approximate local-Nash policy which will be used to measure the accuracy of our planning algorithm.
\begin{definition}
	Given a Markov game $\cM=(\P,r)$, we say policy $(\muhat,\nuhat)$ is an $\epsilon$-approximate local-Nash policy of $\Mcal$ if for all $(h,s)\in [H]\times\cS$, 
	$$\sup_{\mu \in \Delta_{\cA}} (\D_{\mu \times \nuhat_h} Q^{\muhat, \nuhat}_h)(s) - \inf_{\nu \in \Delta_{\cB}} (\D_{\muhat_h \times \nu} Q^{\muhat, \nuhat}_h)(s)\le \epsilon.$$
\end{definition}



Note that finding an $\epsilon$-approximate local-Nash policy for a \emph{known} Markov game is a pure computational problem and requires no sampling at all.

\begin{theorem}\label{thm:rewardfree-explore}
Let $r^1,\ldots,r^N$ be $N$ reward functions chosen independent of the randomness induced by running Algorithm \ref{algorithm:Reward-free-exploration}.
 For any $p \in (0,1]$, choose the exploration bonus $\beta_t$ as in Algrothm~\ref{algorithm:Reward-free-exploration} for $\iota = C\log(SABHTN/p)$ with large absolute constant $C$. Then, with probability at least $1-p$, for all $s\in\cS$, $k\in[K]$, $i\in[N]$ and $(\mu^{ki},\nu^{ki})$ that is $\epsilon_{\rm plan}$-approximate local-Nash for $\widehat{\cM}^{k,i} := (\Phat^k,r^i)$,
$$V^{\dagger,\nu^{ki}}_h(s) - V^{\mu^{ki},\dagger}_h(s) \le \cO\paren{\Vt_h^k(s)+H\epsilon_{\rm plan}}.$$
 \end{theorem}
 
 At a high level, Theorem \ref{thm:rewardfree-explore} claims that the suboptimality of any $\epsilon_{\rm plan}$-approximate local-Nash policy of $\widehat{\cM}^{k,i}$, can be controlled by the corresponding exploration uncertainty $\Vt_1^k(s_1)$ plus the planning error $H\epsilon_{\rm plan}$. Recall that Algorithm \ref{algorithm:Reward-free-exploration} is a zero-reward version of UCB-VI, so we can directly bound $\Vt_1^k(s_1)$ using the regret bound in \cite{azar2017minimax}.
 

\begin{theorem}[UCB-VI]\cite{azar2017minimax} \label{thm:UCB-VI}
For any $p \in (0,1]$, choose the exploration bonus $\beta_t$ as in Algrothm~\ref{algorithm:Reward-free-exploration} for $\iota = C\log(SABHTN/p)$ with large absolute constant $C$. Then, with probability at least $1-p$, 
$$ \sum_{k=1}^{K} \Vt_1^k(s_1) \le \cO(\sqrt{H^4SAK\iota}+H^3S^2A\iota).$$
\end{theorem}

By trivially combining Theorem \ref{thm:rewardfree-explore} with
Theorem \ref{thm:UCB-VI}, we obtain the sample efficiency of Algorithm \ref{algorithm:Reward-free-exploration}.

\begin{corollary}\label{cor:rewardfree-samplecomplex}
	For any $p \in (0,1]$, choose the exploration bonus $\beta_t$ as in Algrothm~\ref{algorithm:Reward-free-exploration} for $\iota = C\log(SABHTN/p)$ with large absolute constant $C$. 
	If we choose $K$ s.t.
	$$
K \ge \Omega(\frac{H^4SAB\iota}{\epsilon_{\rm explore}^2}+\frac{H^3S^2AB\iota}{\epsilon_{\rm explore}}),
$$ 
then, with probability at least $1-p$, for all $i\in[N]$  and 
 $(\mu^{i},\nu^{i})$ that is $\epsilon_{\rm plan}$-approximate local-Nash for $\widehat{\cM}^{k^\star,i} := (\Phat^{k^\star},r^i)$,
	$$V_1^{\dagger,\nu^{i}}(s_1) - V_1^{\mu^{i},\dagger}(s_1) \le \cO\paren{\epsilon_{\rm explore}+H\epsilon_{\rm plan}}.$$
\end{corollary}

Therefore, in order to learn  $\epsilon$-optimal policies for $N$ reward functions simultaneously, $\Omega(H^4SAB\iota/\epsilon^2)$ episodes of exploration suffices,
as long as  the planning algorithm is accurate enough to guarantee $H\epsilon_{\rm plan} \le \epsilon$.

\paragraph{Decoupling planning from exploration.} 
One main advantage of our reward-free framework is that we completely decouple planning from exploration.
Specifically, the only thing we require from the planning algorithm is an approximate local-Nash policy for the input model.
We do not care about how this policy is computed at all.
As a result, we can replace Algorithm \ref{algorithm:Reward-free-planning} by any other approximate planning algorithms and the same theoretical guarantees will still hold. 

In contrast, recent works studying reward-free setting do not enjoy such benefit.
For example, \cite{zhang2020task} requires the samples collected in the exploration phase should be used in a specific incremental manner in the planning phase and 
 \cite{wang2020reward} requires incorporating the exploration bonus into planning.
 
\subsubsection{Planning phase guarantees}
The following theorem shows that Algorithm \ref{algorithm:Reward-free-planning} can compute an approximate local-Nash policy for any input Markov game.
Therefore, we can feed it with the output model of Algorithm \ref{algorithm:Reward-free-exploration} and get a nearly optimal policy for the ground truth model as guaranteed by Corollary  \ref{cor:rewardfree-samplecomplex}.

\begin{theorem}\label{thm:reward-free-plan}
Assume NASH-ZERO-SUM can compute an $\epsilon$-approximate Nash-equilibrium  for any input matrix game.
	Then the output policy of Algorithm \ref{algorithm:Reward-free-planning} is an $\epsilon$-approximate local-Nash policy of the input Markov game.
\end{theorem}

\subsubsection{A lower bound for reward-free Markov games}
\begin{theorem}\label{thm:MG-lowerbound}
There exists an absolute constant $c_1>0$ such that for any $\eps \le c_1$,  there exists a family of Markov games $\mathfrak{M}(\eps)$ satisfying that:  
	for any reward-free algorithm $\mathfrak{A}$ sampling no more than $SABH^2/(10^3\eps^2)$ episodes, there exists a Markov game $\Mcal\in\mathfrak{M}(\eps)$ such that if we run $\mathfrak{A}$ on $\Mcal$, with probability at least $1/3$ it will output a policy  that is at least $2\eps$ suboptimal.
\end{theorem}

Recall in the reward-aware setting, \cite{bai2020near} shows that 
$\tilde{\Theta}(S(A+B)H^6/\epsilon^2)$ episodes suffices for learning an $\epsilon$ optimal policy. 
However, Theorem \ref{thm:MG-lowerbound} claims that in the reward-free setting, the dependence on the number of actions is at least $AB$. 
This result reveals an intrinsic gap between the reward-free and reward-aware settings and also implies that the sample complexity given in  Corollary \ref{cor:rewardfree-samplecomplex} is optimal in terms of $S$, $A$, $B$, $\epsilon$ and at most $H^2$ suboptimal in terms $H$.

Intuitively, the reason \cite{bai2020near} can achieve $A+B$ dependence is that they are doing adaptive sampling utilizing the information of reward. 
However, in the reward-free setting, the reward is agnostic, so in order to find an approximate Nash equilibrium in the planning phase, the algorithm has to collect enough data for all action pairs in the exploration phase, which leads to $AB$ dependence.












